maplab: An Open Framework for Research in Visual-inertial Mapping and Localization

Robust and accurate visual-inertial estimation is crucial to many of today's challenges in robotics. Being able to localize against a prior map and obtain accurate and driftfree pose estimates can push the applicability of such systems even further. Most of the currently available solutions, however, either focus on a single session use-case, lack localization capabilities or an end-to-end pipeline. We believe that only a complete system, combining state-of-the-art algorithms, scalable multi-session mapping tools, and a flexible user interface, can become an efficient research platform. We therefore present maplab, an open, research-oriented visual-inertial mapping framework for processing and manipulating multi-session maps, written in C++. On the one hand, maplab can be seen as a ready-to-use visual-inertial mapping and localization system. On the other hand, maplab provides the research community with a collection of multisession mapping tools that include map merging, visual-inertial batch optimization, and loop closure. Furthermore, it includes an online frontend that can create visual-inertial maps and also track a global drift-free pose within a localization map. In this paper, we present the system architecture, five use-cases, and evaluations of the system on public datasets. The source code of maplab is freely available for the benefit of the robotics research community.

==> sections/a_euroc_evaluation.tex <==
\begin{table}[]
\scriptsize
\centering
\caption{Original table}
\begin{tabular}{@{}l|rr|rr|c@{}}
\toprule
 &
\multicolumn{2}{c|}{\begin{tabular}[c]{c}MH1\\ *LOC: MH2\end{tabular}} & 
\multicolumn{2}{c|}{\begin{tabular}[c]{c}V2-easy\\ *LOC: V2-medium\end{tabular}} &
\multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}CPU load\\ @ 20 Hz\end{tabular}} \\
\cline{2-6}
 & 
\multicolumn{1}{c}{mean} & 
\multicolumn{1}{c|}{RMSE} & 
\multicolumn{1}{c}{mean} & 
\multicolumn{1}{c|}{RMSE} & 
\multicolumn{1}{c}{} \\
\hline
% 1
ROVIO & 
\begin{tabular}[c]{@{}r@{}l@{}} % This @{} seems to remove all the space between the columns, therefore add extra space below.
    0.181 & \,m \\
    0.036 & \,deg
\end{tabular} & 
\begin{tabular}[c]{r@{}l@{}}
    0.210 & \,m \\
    0.038 & \,deg
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.083 & \,m\\ 
    0.977 & \,deg
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.099 & \,m\\ 
    2.451 & \,deg
\end{tabular} &
\begin{tabular}{@{}r@{}c@{}l@{}}
    3.5&$\pm$&0.4\% \\
\end{tabular} \\
\hline
% 2
\begin{tabular}[c]{@{}l@{}}ROVIOLI*\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.063 & \,m\\ 
    0.021 & \,deg
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.081 & \,m\\ 
    0.025 & \,deg
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.062 & \,m\\ 
    1.306 & \,deg
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.068 & \,m\\ 
    2.835 & \,deg
\end{tabular} & 
\begin{tabular}{@{}r@{}c@{}l@{}}
    8.6 & $\pm$ & 0.9\% \\
\end{tabular} \\
\hline
% 3
\begin{tabular}[c]{@{}l@{}}ROVIO+\\ VIWLS\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.031 & \,m\\ 
    0.017 & \,deg
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.032 & \,m\\ 
    0.021 & \,deg
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.020 & \,m\\ 
    0.050 & \,deg
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.021 & \,m\\ 
    0.457 & \,deg
\end{tabular} & 
\begin{tabular}{@{}r@{}c@{}l@{}}
    & -- & \\
\end{tabular} \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[]
\scriptsize
\centering
\caption{Parameter search 1\\
Values:
acc noise density: 2.003e-4 \\
acc bias random walk noise density: 1.25525e-6 \\
gyro noise density: 2.5525e-7 \\
gyro bias random walk noise density: 8.0e-8 \\
}
\label{table:rovio_euroc_evaluation_rmse_new}
\begin{tabular}{@{}l|rr|rr}
\toprule
 &
\multicolumn{2}{c|}{\begin{tabular}[c]{c}MH1\\ *LOC: MH2\end{tabular}} & 
\multicolumn{2}{c}{\begin{tabular}[c]{c}V2-easy\\ *LOC: V2-medium\end{tabular}} \\
\cline{2-5}
 & 
\multicolumn{1}{c}{mean} & 
\multicolumn{1}{c|}{RMSE} & 
\multicolumn{1}{c}{mean} & 
\multicolumn{1}{c}{RMSE} \\
\hline
% 1
ROVIO & 
\begin{tabular}[c]{@{}r@{}l@{}} % This @{} seems to remove all the space between the columns, therefore add extra space below.
    0.123 & \,m \\
\end{tabular} & 
\begin{tabular}[c]{r@{}l@{}}
    0.147 & \,m \\
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.115 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.133 & \,m\\ 
\end{tabular} \\
\hline
% 2
\begin{tabular}[c]{@{}l@{}}ROVIOLI*\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.072 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.097 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.052 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.063 & \,m\\ 
\end{tabular} \\
\hline
% 3
\begin{tabular}[c]{@{}l@{}}ROVIO+\\ VIWLS\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.028 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.030 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.035 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.037 & \,m\\ 
\end{tabular} \\
\hline
% 4
\begin{tabular}[c]{@{}l@{}}ORB-SLAM\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.034 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.038 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.058 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.062 & \,m\\ 
\end{tabular} \\
\hline
% 5
\begin{tabular}[c]{@{}l@{}}ORB-SLAM,\\ real time\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.053 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.073 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.057 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.063 & \,m\\ 
\end{tabular} \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[]
\scriptsize
\centering
\caption{Parameter search 1, front and end of MH1 cut off in evaluation (not in bag)\\
Values:
acc noise density: 2.003e-4 \\
acc bias random walk noise density: 1.25525e-6 \\
gyro noise density: 2.5525e-7 \\
gyro bias random walk noise density: 8.0e-8 \\
\\
Note: ORB-SLAM real-time mode is very inconsistent, so we can also use worse results if necessary
}
\label{table:rovio_euroc_evaluation_rmse_new}
\begin{tabular}{@{}l|rr|rr}
\toprule
 &
\multicolumn{2}{c|}{\begin{tabular}[c]{c}MH1\\ *LOC: MH2\end{tabular}} & 
\multicolumn{2}{c}{\begin{tabular}[c]{c}V2-easy\\ *LOC: V2-medium\end{tabular}} \\
\cline{2-5}
 & 
\multicolumn{1}{c}{median} & 
\multicolumn{1}{c|}{RMSE} & 
\multicolumn{1}{c}{median} & 
\multicolumn{1}{c}{RMSE} \\
\hline
% 1
ROVIO & 
\begin{tabular}[c]{@{}r@{}l@{}} % This @{} seems to remove all the space between the columns, therefore add extra space below.
    0.126 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{r@{}l@{}}
    0.148 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.115 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.133 & \,m\\ 
\end{tabular} \\
\hline
% 2
\begin{tabular}[c]{@{}l@{}}ROVIOLI*\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.069 & \,m \\
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.118 & \,m \\
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.052 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.063 & \,m\\ 
\end{tabular} \\
\hline
% 3
\begin{tabular}[c]{@{}l@{}}ROVIO+\\ VIWLS\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.021 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.023 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.035 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.037 & \,m\\ 
\end{tabular} \\
\hline
% 4
\begin{tabular}[c]{@{}l@{}}ORB-SLAM\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.032 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.042 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.058 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.062 & \,m\\ 
\end{tabular} \\
\hline
% 5
\begin{tabular}[c]{@{}l@{}}ORB-SLAM,\\ real time\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.075 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.093 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.057 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.063 & \,m\\ 
\end{tabular} \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[]
\scriptsize
\centering
\caption{Parameter search 2, optimal parameter (different for MH01 and V201); ORB-SLAM may run BA, even in the end of real-time runs}
\label{table:rovio_euroc_evaluation_rmse_new}
\begin{tabular}{@{}l|rr|rr}
\toprule
 &
\multicolumn{2}{c|}{\begin{tabular}[c]{c}MH1\\ *LOC: MH2\end{tabular}} & 
\multicolumn{2}{c}{\begin{tabular}[c]{c}V2-easy\\ *LOC: V2-medium\end{tabular}} \\
\cline{2-5}
 & 
\multicolumn{1}{c}{median} & 
\multicolumn{1}{c|}{RMSE} & 
\multicolumn{1}{c}{median} & 
\multicolumn{1}{c}{RMSE} \\
\hline
% 1
ROVIO & 
\begin{tabular}[c]{@{}r@{}l@{}} % This @{} seems to remove all the space between the columns, therefore add extra space below.
    0.127 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{r@{}l@{}}
    0.178 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.044 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.064 & \,m\\ 
\end{tabular} \\
\hline
% 2
\begin{tabular}[c]{@{}l@{}}ROVIOLI*\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.049 & \,m \\
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.082 & \,m \\
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.039 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.057 & \,m\\ 
\end{tabular} \\
\hline
% 3
\begin{tabular}[c]{@{}l@{}}ROVIO+\\ VIWLS\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.029 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.036 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.026 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.027 & \,m\\ 
\end{tabular} \\
\hline
% 4
\begin{tabular}[c]{@{}l@{}}ORB-SLAM\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.032 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.031 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.052 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.056 & \,m\\ 
\end{tabular} \\
\hline
% 5
\begin{tabular}[c]{@{}l@{}}ORB-SLAM,\\ real time\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.034 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.073 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.057 & \,m\\ 
\end{tabular} & 
\begin{tabular}[c]{@{}r@{}l@{}}
    0.063 & \,m\\ 
\end{tabular} \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[]
\scriptsize
\centering
\caption{General timing, MH1 (*LOC:MH2) @ 20Hz}
\begin{tabular}{@{}l|r|c}
\toprule
    & Frame processing time [ms] & CPU load \\
\hline
    with localization* & 
    234$\pm$24.9 & 
    \begin{tabular}{@{}r@{}c@{}l@{}}
        105.3\%&$\pm$&14.8\% \\
    \end{tabular} \\
\hline
    without localization & 
    237$\pm$26 & 
    \begin{tabular}{@{}r@{}c@{}l@{}}
        56.2\%&$\pm$&7.7\% \\
    \end{tabular} \\
\hline
    ORB-SLAM & 
    67 & 
    \begin{tabular}{@{}r@{}c@{}l@{}}
        223.5\%&$\pm$&43.9\% \\
    \end{tabular} \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[]
\scriptsize
\centering
\caption{Detailed timing ROVIOLI with localization @ 20Hz}
\begin{tabular}{@{}l|r}
\toprule
    & Processing time [ms] \\
\hline
    ROVIO update & 22.2$\pm$13.9 \\
    Feature tracking & 18.8$\pm$6.5 \\
    Localization & 18.8$\pm$3.8 \\
    ROVIO localization update & 1.7$\pm$0.1 \\
    Map building & 3.1$\pm$0.2 \\
\hline
    \textbf{Total} & \textbf{234$\pm$24.9} \\
\bottomrule
\end{tabular}
\end{table}

==> tables/commands.tex <==
\begin{table*}[]
\centering
\scriptsize
\caption{Quick reference of the most commonly used commands in the maplab console.}
\label{framework:core_table}
\begin{tabular}{p{2.5cm} p{14.5cm}}
\hline
\multicolumn{2}{l}{\textbf{Basic commands}}                                                                                                                                                                                                                                                                                                                                    \\ \hline
\texttt{help}                 & Displays reference for all the commands.                                                                                                                                                                                                                                                                                 \\
\texttt{load, save}                 & Load/save a map from disk.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\
\texttt{map\_stats}           & Prints statistics of the trajectories present in the map.                                                                                                                                                                                                                                                                         \\
\texttt{list}                 & Lists all maps present in the system.                                                                                                                                                                                                                                                                                             \\
\texttt{select}               & Selects the currently active map. All algorithms operate on the currently active map.                                                                                                                                                                                                                                             \\ \hline
\multicolumn{2}{l}{\textbf{Optimization}}                                                                                                                                                                                                                                                                                                                                \\ \hline
\texttt{rtl}                  & Retriangulates the 3d positions of all landmarks present in the map. Simultaneously, it also detects landmarks that are not well constrained -- they are marked as \textit{bad} and ignored by subsequent commands.                                                                                                             \\
\texttt{optv}                 & Performs a visual-only least-squares optimization of the map. The inertial data is not used. Useful for tuning the system.                                                                                                                                                                     \\
\texttt{optvi}                & Performs a visual-inertial least-squares optimization of the map. A major batch optimization algorithm used to refine the quality of the map coming from ROVIOLI.                                                                                                                                                                 \\
\texttt{relax}                & Performs posegraph relaxation using loop closure edges. Relaxation is particularly useful to correct for drift of the visual-inertial estimator. \\ \hline
\multicolumn{2}{l}{\textbf{Map anchoring}}                                                                                                                                                                                                                                                                                                                                \\ \hline
\texttt{anchor\_all\_missions}    & Attempts to anchor all trajectories in the global coordinate frame. Useful for creating a consistent reconstruction from multiple mapping sessions.                                                                                                                                                                               \\ \hline
\multicolumn{2}{l}{\textbf{Map sparsification}}                                                                                                                                                                                                                                                                                                                              \\ \hline
\texttt{kfh}                  & Keyframes the vertices of the map based on a set of heuristics. As a result, it reduces the computational requirements of algorithms and the storage footprint of the map.                                                                                                                                                        \\
\texttt{summary\_map}         & Summarizes the landndmarks of the map and stores the result as a compact localization map that can be loaded by ROVIOLI later on.                                                                                                                                                                                                 \\ \hline
\multicolumn{2}{l}{\textbf{Loopclosure}}                                                                                                                                                                                                                                                                                                                                     \\ \hline
\texttt{lc}                   & Searches for loopclosures between all trajectories pairwise. Merges duplicated landmarks. Additionally, it introduces loopclosure edges that can be used for posegraph relaxation.                                                                                                                                                \\
\texttt{eloc}                 & Evaluates the localization between a set of database trajectories and a query trajectory.                                                                                                                                                          \\ \hline
\multicolumn{2}{l}{\textbf{Dense reconstruction}}
            \\ \hline
\texttt{mdr}                  & Rectification-based, 3d reconstruction~\cite{ThesisJaeger2015} of monocular and stereo images images attached to the VI-map.
            \\
\texttt{improve\_depth\_maps} & Fuses and filters covisible depth maps.
            \\
\texttt{export\_for\_pmvs}    & Exports the localized images attached to the vi-map and the covisibility graph to the input format of CMVS/PMVS2~\cite{Furu:2010,Furu:2010:PMVS}, a patch-based multi-view stereo reconstruction framework. This allows for dense, high-quality 3d reconstructions.
            \\
\texttt{depth\_fusion}        & Fuses all depth maps attached to the VI-map in a TSDF voxel grid~\cite{oleynikova2016voxblox}, creates a 3d reconstruction and exports the surface mesh as a PLY file.
            \\ \hline
\multicolumn{2}{l}{\textbf{Visualization}}                                                                                                                                                                                                                                                                                                                                   \\ \hline
\texttt{visualize}            & Visualizes the current state of the map by publishing ROS messages with RViz markers.                                                                                                                                                                                                                                             \\
\texttt{plot\_vi\_states}                 & Shows a plot of the visual-inertial states stored in vertices (pose, IMU biases, velocity) over time. This might be useful for understanding the IMU forward propagation or tuning the IMU bias and noise parameters.                                                                                                           \\ \hline
\end{tabular}
\end{table*}

==> tables/unused_summarization.tex <==
\begin{comment}
\begin{table}[]
\scriptsize
\centering
\caption{Influence of landmark summarization and keyframing on the localization map size. 
%
Keyframing removes vertices including very expensive vertex-landmark associations.
%
This permits to make very considerable map size savings.}
\label{table:summarization_sizes}
\begin{tabular}{cl|rrr}
\toprule
keyframe             & summarize & \# vertices            & \# landmarks & map size {[}MB{]} \\ \hline
\multirow{7}{*}{no}  & 0         & \multirow{7}{*}{6,258} & 18,316       & 34.559            \\
                     & 0.25      &                        & 12,972       & 32.009            \\
                     & 0.5       &                        & 8,824        & 29.217            \\
                     & 0.75      &                        & 4,529        & 24.028            \\
                     & 0.9       &                        & 1,818        & 17.619            \\
                     & 0.95      &                        & 899          & 12.203            \\
                     & 0.98      &                        & 349          & 6.707             \\ \hline
\multirow{7}{*}{yes} & 0         & \multirow{7}{*}{760}   & 16,088       & 3.740             \\
                     & 0.25      &                        & 13,097       & 3.528             \\
                     & 0.5       &                        & 9,148        & 3.209             \\
                     & 0.75      &                        & 4,570        & 2.602             \\
                     & 0.9       &                        & 1,822        & 1.837             \\
                     & 0.95      &                        & 906          & 1.214             \\
                     & 0.98      &                        & 358          & 0.712             \\ \bottomrule
\end{tabular}
\end{table}
\end{comment}

\begin{comment}
\begin{tabular}{ll|lllll}
summarization & keyframing & \# vertices & \# landmarks & ILP loc. map size {[}MB{]} & \begin{tabular}[c]{@{}l@{}}ILP recall \\ (@100\% precision)\end{tabular} & Random recall \\ \hline
-             & no         & 6258        & 18316        & 34.559                     & 0.6050                                                                   & 0.6050        \\
-             & yes        & 760         & 16088        & 3.740                      & 0.5221                                                                   & 0.5221        \\
0.75          & no         & 6258        & 12972        & 32.009                     & 0.6057                                                                   & 0.0737        \\
0.5           & no         & 6258        & 8824         & 29.217                     & 0.5931                                                                   & 0.0323        \\
0.25          & no         & 6258        & 4529         & 24.028                     & 0.6015                                                                   & 0.0063        \\
0.1           & no         & 6258        & 1818         & 17.619                     & 0.5523                                                                   & 0             \\
0.05          & no         & 6258        & 899          & 12.203                     & 0.4764                                                                   & 0             \\
0.02          & no         & 6258        & 349          & 6.707                      & 0.2396                                                                   & 0             \\
0.75          & yes        & 760         & 13097        & 3.528                      & 0.5305                                                                   & 0.1419        \\
0.5           & yes        & 760         & 9148         & 3.209                      & 0.5242                                                                   & 0.1103        \\
0.25          & yes        & 760         & 4570         & 2.602                      & 0.5102                                                                   & 0.0070        \\
0.1           & yes        & 760         & 1822         & 1.837                      & 0.4877                                                                   & 0             \\
0.05          & yes        & 760         & 906          & 1.214                      & 0.3956                                                                   & 0             \\
0.02          & yes        & 760         & 358          & 0.712                      & 0.2297                                                                   & 0            
\end{tabular}
\end{comment}
